What Can I Do Here? Learning New Skills by Imagining Visual Affordances

A generalist robot equipped with learned skills must be able to perform many tasks in many different environments. However, zero-shot generalization to new settings is not always possible. When the robot encounters a new environment or object, it may need to finetune some of its previously learned skills to accommodate this change. But crucially, previously learned behaviors and models should still be suitable to accelerate this relearning. In this paper, we aim to study how generative models of possible outcomes can allow a robot to learn visual representations of affordances, so that the robot can sample potentially possible outcomes in new situations, and then further train its policy to achieve those outcomes. In effect, prior data is used to learn what kinds of outcomes may be possible, such that when the robot encounters an unfamiliar setting, it can sample potential outcomes from its model, attempt to reach them, and thereby update both its skills and its outcome model. This approach, visuomotor affordance learning (VAL), can be used to train goal-conditioned policies that operate on raw image inputs, and can rapidly learn to manipulate new objects via our proposed affordance-directed exploration scheme. We show that VAL can utilize prior data to solve real-world tasks such drawer opening, grasping, and placing objects in new scenes with only five minutes of online experience in the new scene.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> texs/fig_samples.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{0.12\textwidth}
        \center
        \includegraphics[height=0.99\textwidth]{imgs/views/simb_view.jpeg}
        \vspace{0.02cm}
        
        \includegraphics[width=0.99\textwidth]{imgs/views/sima_view.jpeg}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}[b]{0.14\textwidth}
        % \center
        \begin{flushright}
        % \textbf{Samples}
        
        Initial Image
        
        \vspace{0.35cm}
        
        CVQVAE (Ours)
        
        \vspace{0.35cm}
        
        CCVAE
        
        \vspace{0.35cm}
        
        CBiGAN
        
        \vspace{0.35cm}
        
        VAE
        
        \vspace{1.1cm}
        
        % BiGAN
        \end{flushright}
        
        % \textbf{Reconstructions}
        
        % Image
        
        % CVQVAE (Ours)
        
        % CCVAE
        
        % CBiGAN
        
        % VAE
        
        % BiGAN
        
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \center
        
        \scalebox{1.4}{
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s1.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s2.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s3.png} } \hspace{-12px}
                % \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s4.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s5.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/f1.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/f2.png} } \hspace{-12px}
% \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/f3.png} }
            }
    
        \hspace{0.5cm}\textcolor{green}{\rule{3cm}{2px}} \hspace{0.5cm} \textcolor{red}{\rule{1cm}{2px}}
        
        Sim Setting A
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \center
        
            \scalebox{1.4}{
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/s1.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/s3.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/s2.png} } \hspace{-12px}
                % \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/s4.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/s5.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/f1.png} } \hspace{-12px}
                \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim2/f2.png} } \hspace{-12px}
% \adjustbox{trim=0 16 0 0,clip} { \includegraphics[width=0.1\textwidth]{imgs/samples/sim1/f3.png} }
            }
    
        \hspace{0.5cm}\textcolor{green}{\rule{3cm}{2px}} \hspace{0.5cm} \textcolor{red}{\rule{1cm}{2px}}
        
        Sim Setting B
    \end{subfigure}
    \caption{Left: randomly sampled work spaces from our simulated multi-task environment. Right: samples on test environments in simulation. In each column, the top image is the conditioning image $s_0$ and the images below are conditional sampled image. Successful samples for our affordance model are highlighted in green, and show the potential outcome of a behavior. Failure modes are highlighted in red, and lack diversity or alter an object's geometry or color.  }
    \label{fig:samples}
    \vspace{-0.5cm}
\end{figure*}

==> texs/fig_views.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.99\linewidth}
        \center
        \includegraphics[height=0.3\textwidth]{imgs/views/sima_view.jpeg}
        \includegraphics[height=0.3\textwidth]{imgs/views/simb_view.jpeg}
    \end{subfigure}

    \caption{Randomly sampled environments from the two simulation settings: simulation A on the left is used to study grasping and relocating novel objects, and simulation setting B on the right is used to study learning distinct skills in single environment.}
    \label{fig:env_views}
    \vspace{-0.5cm}
\end{figure}

==> texs/paper_specific_commands_and_packages.tex <==
\usepackage{xspace}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{subcaption}
\usepackage{floatrow}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{xcolor}
\usepackage{appendix}
\usepackage[normalem]{ulem}
\def\appendixautorefname{Appendix}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\algorithmautorefname{Algorithm}
%\newcommand*{\Appendixautorefname}{Appendix}




% From https://tex.stackexchange.com/questions/149807/autoref-subsections-in-appendix
% begin appendix autoref patch [\autoref subsections in appendix](https://tex.stackexchange.com/questions/149807/autoref-subsections-in-appendix)
\usepackage{etoolbox}
\makeatletter
\patchcmd{\hyper@makecurrent}{%
    \ifx\Hy@param\Hy@chapterstring
        \let\Hy@param\Hy@chapapp
    \fi
}{%
    \iftoggle{inappendix}{%true-branch
        % list the names of all sectioning counters here
        \@checkappendixparam{chapter}%
        \@checkappendixparam{section}%
        \@checkappendixparam{subsection}%
        \@checkappendixparam{subsubsection}%
        \@checkappendixparam{paragraph}%
        \@checkappendixparam{subparagraph}%
    }{}%
}{}{\errmessage{failed to patch}}

\newcommand*{\@checkappendixparam}[1]{%
    \def\@checkappendixparamtmp{#1}%
    \ifx\Hy@param\@checkappendixparamtmp
        \let\Hy@param\Hy@appendixstring
    \fi
}
\makeatletter

\newtoggle{inappendix}
\togglefalse{inappendix}

\apptocmd{\appendix}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
\apptocmd{\subappendices}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}







\newcommand\comment[1]{\textcolor{red}{#1}}
\newcommand\strike{\bgroup\markoverwith{\textcolor{red}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon}
\definecolor{darkgreen}{RGB}{0,180,56}
\newcommand{\NEW}[1]{\textcolor{darkgreen}{#1}}
% \newcommand{\NEW}[1]{\textcolor{Green}{#1}}
% \newcommand{\strike}[1]{\vphantom{#1}}
% \newcommand{\NEW}[1]{#1}
\newcommand{\sampleN}{\stackrel{N}{\sim}}
\newcommand{\fcaption}[1]{\caption{{\footnotesize{#1}}}}


\newcommand{\uniform}[1]{\text{Uniform}[#1]}
\newcommand{\simple}{\text{na\"{\i}ve}}

\newcommand{\pap}{{\theta}}
\newcommand{\papprox}{{p_\pap}}
\newcommand{\papproxt}{{p_{\pap_t}}}
\newcommand{\papproxtt}{{p_{\pap_{t+1}}}}
\newcommand{\pspg}{p(\SF \mid \pg)}
\newcommand{\pspgt}{p(\SF \mid \pgt)}
\newcommand{\pspgtt}{p(\SF \mid \pgtt)}
\newcommand{\z}{{\mathbf{z}}}
\newcommand{\wt}{{w_{t, \alpha}}}



% Sets
\newcommand{\FullSpaceDim}{n}
\newcommand{\FullSpace}{{\mathbb{R}^\FullSpaceDim}}
\newcommand{\Imgs}{{\mathcal{S}}}
\newcommand{\nImgs}{{\overline{\gS}}}
\newcommand{\Ss}{{\mathcal{S}}}
\newcommand{\As}{{\mathcal{A}}}
\newcommand{\Gs}{{\mathcal{G}}}
\newcommand{\ImgSets}{{\sA}}
\newcommand{\Rnn}{{\sR^{n\times n}}}
\newcommand{\validq}{\mathcal{Q}}

% MDP
\newcommand{\G}{\mathbf{G}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\SF}{\mathbf{S}}
\newcommand{\stf}{\mathbf{s}}
\newcommand{\St}{\mathbf{S}}
\newcommand{\st}{\mathbf{s}}
\newcommand{\zt}{\mathbf{z}}
\newcommand{\At}{\mathbf{A}}
\newcommand{\at}{\mathbf{a}}
\newcommand{\dyn}{\rho(\st_{t+1} \mid \st_t, \at_t)}

\newcommand{\MI}{I(\G, \SF)}
\newcommand{\HG}{\gH(\G)}
\newcommand{\HGS}{\gH(\G \mid \SF)}
\newcommand{\entropy}{\mathcal{H}}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\SFLoss}{\mathcal{L}^\text{SF}}
\newcommand{\Lossq}{\mathcal{L}_\text{SKEW}}
\newcommand{\Lossp}{\mathcal{L}_\text{FIT}}
\newcommand{\pstate}{{p(\St \mid \pg)}}
\newcommand{\pstatet}{{p(\St \mid \pgt)}}
\newcommand{\pstatett}{{p(\St \mid \pgtt)}}

\newcommand{\U}{{U_\Imgs}}
\newcommand{\UA}{{U_\gA}}
\newcommand{\dynamics}{{p_\mathrm{dyn}}}
% Generative model
\newcommand{\pgparam}{{\phi}}
\newcommand{\pgparamt}{{\pgparam_t}}
\newcommand{\pgparamtt}{{\pgparam_{t+1}}}
%\newcommand{\pg}{{p_g}}
%\newcommand{\pgt}{{p_{g_t}}}
%\newcommand{\pgtt}{{p_{g_{t+1}}}}
\newcommand{\pg}{{p_\pgparam}}
\newcommand{\pgt}{{p_{\pgparam_t}}}
\newcommand{\pgtt}{{p_{\pgparam_{t+1}}}}
% Empirical distribution
\newcommand{\pe}{{p_\text{emp}}}
\newcommand{\pet}{{p_{\text{emp}_t}}}
\newcommand{\pes}[1]{{p_{\text{emp}_{#1}}}}
\newcommand{\pett}{{p_{\text{emp}_{t+1}}}}
% Weighted empirical distribution
\newcommand{\pwe}{\textcolor{red}{\bar {q}}}
% Skewed distribution
\newcommand{\pskewed}{{p_{\text{skewed}}}}
\newcommand{\pskewedt}{{p_{\text{skewed}_t}}}
\newcommand{\pskeweds}[1]{{p_{\text{skewed}_{#1}}}}
\newcommand{\pskewedtt}{{p_{\text{skewed}_{t+1}}}}
% For proof
\newcommand{\pt}{{p_\theta}}
\newcommand{\ptt}{{p_\theta^t}}
\newcommand{\htt}{{\gH_\theta^t}}
\newcommand{\replay}{\mathcal{R}}

%% Notation switches
\newcommand{\qe}{{\hat {q}}}
% Weighted empirical distribution
\newcommand{\qwe}{{\bar {q}}}

\newcommand{\inX}{{\G}}
\newcommand{\outX}{{\SF}}
\newcommand{\x}{x}

\newcommand{\DTV}{D_\mathrm{TV}}
\newcommand{\NOTE}[1]{\textcolor{red}{(#1)}}
\newcommand{\TODO}[1]{\textcolor{red}{(TODO: #1)}}
\newcommand{\METHOD}{Advantage Weighted Actor Critic\xspace}
\newcommand{\METHODmath}{\text{Skew-Fit}}
\newcommand{\METHODRIG}{Skew-Fit with RIG\xspace}
\newcommand{\CONTRACTIVE}{contractive\xspace}
\newcommand{\ESTABLE}{$\epsilon$-stable}
\newcommand{\dynop}{{\mathcal{F}_\mathrm{dyn}}}
\newcommand{\UB}{\mathcal{L}}
\newcommand{\error}{e}

% From https://tex.stackexchange.com/questions/422/how-do-i-repeat-a-theorem-number
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{assumption}{Assumption}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{property}[theorem]{Property}
\newtheorem{definition}[theorem]{Definition}
\def\assumptionref#1{assumption~\ref{#1}}
\def\Assumptionref#1{Assumption~\ref{#1}}
\def\lemmaref#1{lemma~\ref{#1}}
\def\Lemmaref#1{Lemma~\ref{#1}}
\def\theoremref#1{theorem~\ref{#1}}
\def\Theoremref#1{Theorem~\ref{#1}}
\def\propertyref#1{property~\ref{#1}}
\def\Propertyref#1{Property~\ref{#1}}


\newcommand{\bigO}{\mathcal{O}}

\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{multicol}
\usepackage{enumitem}

